MOANA: Multi-Radar Dataset for Maritime Odometry and Autonomous Navigation Application

Maritime environmental sensing requires overcoming challenges from complex conditions such as harsh weather, platform perturbations, large dynamic objects, and the requirement for long detection ranges. While cameras and LiDAR are commonly used in ground vehicle navigation, their applicability in maritime settings is limited by range constraints and hardware maintenance issues. Radar sensors, however, offer robust long-range detection capabilities and resilience to physical contamination from weather and saline conditions, making it a powerful sensor for maritime navigation. Among various radar types, X-band radar is widely employed for maritime vessel navigation, providing effective long-range detection essential for situational awareness and collision avoidance. Nevertheless, it exhibits limitations during berthing operations where near-field detection is critical. To address this shortcoming, we incorporate W-band radar, which excels in detecting nearby objects with a higher update rate. We present a comprehensive maritime sensor dataset featuring multi-range detection capabilities. This dataset integrates short-range LiDAR data, medium-range W-band radar data, and long-range X-band radar data into a unified framework. Additionally, it includes object labels for oceanic object detection usage, derived from radar and stereo camera images. The dataset comprises seven sequences collected from diverse regions with varying levels of \bl{navigation algorithm} estimation difficulty, ranging from easy to challenging, and includes common locations suitable for global localization tasks. This dataset serves as a valuable resource for advancing research in place recognition, odometry estimation, SLAM, object detection, and dynamic object elimination within maritime environments. Dataset can be found at https://sites.google.com/view/rpmmoana.

==> admin/cover_letter.tex <==
We would like to submit the following manuscript for consideration for the IJRR dataset paper. We have conducted a dataset that firstly incorporates multiple radars with different bandwidths in maritime environments. While traditional marine radars using X-band wavelengths face limitations in short-range detection near port areas, our inclusion of W-band radar addresses this gap by providing superior short-distance perception capabilities, outperforming even LiDAR in maritime scenarios.

Our dataset captures spatio-temporal diversity across various maritime scenarios. Comprising 8 sequences with diverse scenes, it provides ground-truth trajectories for navigation and object annotations for each radar modality. Our benchmark results demonstrate the need for research into complementary radar setups for SLAM in oceanic areas.

We are extending the foundational work of previous IJRR dataset papers [1, 2] by targeting multi-modal applications in maritime settings. Unlike existing datasets, ours uniquely incorporates W-band radar in both open-water scenes and near-port areas, introducing a variety of maritime navigational challenges.

[1] Burnett K, Yoon DJ, Wu Y, Li AZ, Zhang H, Lu S, Qian J, Tseng WK, Lambert A, Leung KY, Schoellig AP and Barfoot TD (2023) Boreas: A multi-season autonomous driving dataset. Intl. J. of Robot. Research 42(1-2):33-42.
[2] Chung D, Kim J, Lee C and Kim J (2023) Pohang canal dataset: A multimodal maritime dataset for autonomous navigation in restricted waters. Intl. J. of Robot. Research 42(12): 1104–1114.
